A Faithful Semantics for Generalised Symbolic Trajectory Evaluation

Generalised Symbolic Trajectory Evaluation (GSTE) is a high-capacity formal verification technique for hardware. GSTE uses abstraction, meaning that details of the circuit behaviour are removed from the circuit model. A semantics for GSTE can be used to predict and understand why certain circuit properties can or cannot be proven by GSTE. Several semantics have been described for GSTE. These semantics, however, are not faithful to the proving power of GSTE-algorithms, that is, the GSTE-algorithms are incomplete with respect to the semantics. The abstraction used in GSTE makes it hard to understand why a specific property can, or cannot, be proven by GSTE. The semantics mentioned above cannot help the user in doing so. The contribution of this paper is a faithful semantics for GSTE. That is, we give a simple formal theory that deems a property to be true if-and-only-if the property can be proven by a GSTE-model checker. We prove that the GSTE algorithm is sound and complete with respect to this semantics.

==> clock.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% File: clock.tex
% Date: April 10, 2001
% Author: Oliver Corff
% (c) 2001 Ulaanbaatar, Macau, Berlin
%
% A package for providing graphical
% clocks to TeX- and LaTeX-users.
%
% Usage: \input clock
%
% No options.
%
% NB: This file does not require LaTeX2e!
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Size definitions
%
\ifx\LaTeXclock\undefined
	\font\myclockfont clock
	\font\mybigclockfont clock at 24pt
	%
	\def\clockfont{\let\clockfont\myclockfont}
	\def\bigclockfont{\let\clockfont\mybigclockfont}
\fi

\ifx\TeXclock\undefined
	\def\TeXclock{}
	\catcode`@ 11
\else
	\endinput
\fi

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Variables
%
	\newcount\time@in@minutes
	\newcount\floor@minutes
	\newcount\hour@minutes
	\newcount\text@hours
	\newcount\text@minutes
	\newcount\my@minute
	\newcount\my@minutes
	\newcount\my@hour
	\newcount\ClockStyle		% one of 1 2 3 4
	\global\newif\ifClockFrame	% one of true false
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Time Calculations
%
\def\calc@hours{%
	\time@in@minutes=\time
	\text@hours=\time@in@minutes
	\divide\text@hours by 60 }

\def\texthours{%
	\calc@hours
	\the\text@hours }

\def\calc@minutes{%
	\calc@hours
	\floor@minutes=\text@hours
	\multiply\floor@minutes by 60
	\text@minutes=\time@in@minutes
	\advance\text@minutes-\floor@minutes }

\def\textminutes{%
	\calc@minutes
	\ifnum\text@minutes<10 0\fi
	\the\text@minutes}

\def\texttime{\texthours:\textminutes}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Display Operations
%
\def\show@clock#1#2{%
	{\clockfont %
	\char#1\kern-1.00ex \char#2%	% Print hours and minutes!
	\advance\ClockStyle by 48	% Build dial
	\ifnum\ClockStyle>48
		\kern-1ex\char\ClockStyle %
	\fi
	\ifClockFrame \kern-1ex\char48 \fi
	}}

\def\calc@movement{%
	\ifnum\my@hour>11 \advance\my@hour by -12 \fi
	\multiply\my@hour by 5
	\my@minutes=\my@minute
	\divide\my@minutes by 12
	\advance\my@hour by \my@minutes
	\advance\my@hour by 128
	\advance \my@minute by 64
	}

\def\clock#1#2{%
	\my@hour#1\my@minute#2%
	\calc@movement
	\show@clock{\my@hour}{\my@minute}}


\def\clocktime{%
	\calc@minutes % Calls \calc@hours
	\clock{\text@hours}{\text@minutes}
	}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Initial Settings
%
\ClockStyle=1
\ClockFramefalse
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% Some Housekeeping...
%
\ifx\LaTeXclock\undefined
	\catcode`@ 12
\fi

